Context-Informed Machine Translation of Manga using Multimodal Large Language Models

Due to the significant time and effort required for handcrafting translations, most manga never leave the domestic Japanese market. Automatic manga translation is a promising potential solution. However, it is a budding and underdeveloped field and presents complexities even greater than those found in standard translation due to the need to effectively incorporate visual elements into the translation process to resolve ambiguities. In this work, we investigate to what extent multimodal large language models (LLMs) can provide effective manga translation, thereby assisting manga authors and publishers in reaching wider audiences. Specifically, we propose a methodology that leverages the vision component of multimodal LLMs to improve translation quality and evaluate the impact of translation unit size, context length, and propose a token efficient approach for manga translation. Moreover, we introduce a new evaluation dataset -- the first parallel Japanese-Polish manga translation dataset -- as part of a benchmark to be used in future research. Finally, we contribute an open-source software suite, enabling others to benchmark LLMs for manga translation. Our findings demonstrate that our proposed methods achieve state-of-the-art results for Japanese-English translation and set a new standard for Japanese-Polish.

==> sections/app-copy.tex <==
\section{Copyright}
\label{sec:copyright}
After confirming with the publisher of the Polish translation that the copyright for the translation had expired in Poland, we obtained second-hand physical copies of both volumes and manually transcribed the translations, as the publisher no longer possessed the data.
%
In an effort to legally obtain original Japanese manga scans for evaluation, we reached out to seven of the largest Japanese publishers. 
%
All these publishers have websites that allow users to buy electronic versions of manga and offer free previews of the first few chapters for many titles. 
%
We inquired about the possibility of using these free previews for research and redistributing them as datasets for future works, emphasizing that they would be used only for evaluation and not for training machine learning models.
%
Unfortunately, all the publishers refused to permit the use and redistribution of that data, citing reasons such as having a policy of not accepting personal requests (three publishers) or not engaging in this type of data sharing at all (four publishers).
